Optimizing transient gas network control for challenging real-world instances using MIP-based heuristics

Optimizing the transient control of gas networks is a highly challenging task. The corresponding model incorporates the combinatorial complexity of determining the settings for the many active elements as well as the non-linear and non-convex nature of the physical and technical principles of gas transport. In this paper, we present the latest improvements of our ongoing work to solve this problem for real-world, large-scale problem instances: By adjusting our mixed-integer non-linear programming model regarding the gas compression capabilities in the network, we reflect the technical limits of the underlying units more accurately while maintaining a similar overall model size. In addition, we introduce a new algorithmic approach that is based on splitting the complexity of the problem by first finding assignments for discrete variables and then determining the continuous variables as locally optimal solution of the corresponding non-linear program. For the first task, we design multiple different heuristics based on concepts for general time-expanded optimization problems that find solutions by solving a sequence of sub-problems defined on reduced time horizons. To demonstrate the competitiveness of our approach, we test our algorithm on particularly challenging historic demand scenarios. The results show that high-quality solutions are obtained reliably within short solving times, making the algorithm well-suited to be applied at the core of time-critical industrial applications.

==> commands.tex <==
\RequirePackage{xspace}
\RequirePackage{accents}

%%-------------------------------------------------------------
%% Abbreviations
%%-------------------------------------------------------------
\newcommand{\myie}{i.e.}
\newcommand{\myIe}{I.e.}
\newcommand{\myeg}{e.g.}
\newcommand{\myst}{s.t.\ }
\newcommand{\myWlog}{W.l.o.g.\ }
\newcommand{\mywlog}{w.l.o.g.\ }
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

% nice underbar, needs 'accents' package
%\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
\newcommand{\ubar}[1]{\underaccent{\bar}{{#1}}}

\newcommand{\ub}[1]{\ensuremath{\bar{#1}}\xspace}
\newcommand{\lb}[1]{\ensuremath{\ubar{#1}}\xspace}

\newcommand{\powerset}{\ensuremath{\mathcal{P}}\xspace}
% set of halfspaces representing the faces of some polytope (compressor config polytope, tv bound polytope, etc.)
\newcommand{\setFacets}[1]{\ensuremath{\mathcal{H}_{#1}}\xspace}

%%----------------------------------------------------------
%% all used mathcal letters
%%----------------------------------------------------------
% A - arcs
% C - (aux) compressor (station) configurations
% F - flow directions
% G - fence groups
% H - configuration facets(hyperplanes)
% I - network stations
% M - machines (maybe unify with U?)
% O - operation modes
% P - power set
% Q - valid operation mode/flowdirection combinations
% S - Simple states
% T - time steps
% U - units (maybe unify with M?)
% V - vertices
% W - flow direction conditions
% Z - aux compressor configuration conflicts

%%-----------------------------------------------------------
%% Graph
%%----------------------------------------------------------
\newcommand{\graph}{\ensuremath{G}\xspace}
\newcommand{\generalGraph}{\ensuremath{\graph=(\setVertices,\setArcs)}\xspace}
\newcommand{\netmodelGraph}{\ensuremath{\graph=(\setVertices,\setPipes \cup \setRegulators \cup \setValves \cup \setArtificialLinks)}\xspace}

% nodes
\newcommand{\setVertices}{\ensuremath{\mathcal{V}}\xspace}
\newcommand{\setVerticesAll}{\ensuremath{\setVertices = \setBoundaryNodes \cup \setInnerNodes}\xspace}
\newcommand{\setEntries}{\ensuremath{\setVertices^{+}}\xspace}
\newcommand{\setExits}{\ensuremath{\setVertices^{-}}\xspace}
\newcommand{\setBoundaryNodes}{\ensuremath{\setVertices^\mathrm{b}}\xspace}
\newcommand{\setBoundaryNodesAll}{\ensuremath{\setEntries \cup \setExits}\xspace}
\newcommand{\setInnerNodes}{\ensuremath{\setVertices^{0}}\xspace}
\newcommand{\setFenceNodes}{\ensuremath{\setVertices^{\mathrm{fn}}}\xspace}
\newcommand{\setFenceNodesNaviStation}[1]{\ensuremath{\setFenceNodes_{#1}}\xspace}
\newcommand{\setArtificialNodes}{\ensuremath{\setVertices^{\mathrm{ar}}}\xspace}
\newcommand{\setArtificialNodesNaviStation}[1]{\ensuremath{\setArtificialNodes_{#1}}\xspace}

% arcs
\newcommand{\setArcs}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\setArcsAllStationModel}{\ensuremath{\setArcs = \setPipes \cup \setValves \cup \setResistors \cup \setRegulators \cup \setCompressorStations}\xspace}
\newcommand{\setPipes}{\ensuremath{\setArcs^{\mathrm{pi}}}\xspace}
\newcommand{\setRegulators}{\ensuremath{\setArcs^{\mathrm{rg}}}\xspace}
\newcommand{\setValves}{\ensuremath{\setArcs^{\mathrm{va}}}\xspace}
\newcommand{\setValvesNS}{\ensuremath{\setArcs^{\mathrm{va-s}}}\xspace}
\newcommand{\setValvesFN}{\ensuremath{\setArcs^{\mathrm{vaFn}}}\xspace}
\newcommand{\setValvesOrig}{\ensuremath{\setArcs^{\mathrm{vaOr}}}\xspace}
\newcommand{\setResistors}{\ensuremath{\setArcs^{\mathrm{rs}}}\xspace}
\newcommand{\setCompressorStations}{\ensuremath{\setArcs^{\mathrm{cs}}}\xspace}

% station model specific arcs
\newcommand{\setRegulatorsControllable}{\ensuremath{\setArcs^{\mathrm{rg-c}}}\xspace}
\newcommand{\setRegulatorsNonControllable}{\ensuremath{\setArcs^{\mathrm{rg-nc}}}\xspace}
\newcommand{\setRegulatorsNonControllableActive}{\ensuremath{\setArcs^{\mathrm{rg-nca}}}\xspace}
\newcommand{\setRegulatorsNonControllableFixed}{\ensuremath{\setArcs^{\mathrm{rg-ncf}}}\xspace}
\newcommand{\setRegulatorsNonControllableAll}{\ensuremath{\setRegulatorsNonControllable := \setRegulatorsNonControllableActive\cup\setRegulatorsNonControllableFixed}\xspace}

% special compressor station sets
\newcommand{\setCompressorUnits}{\ensuremath{\mathcal{U}}\xspace}
\newcommand{\setCompressorUnitsI}[1]{\ensuremath{\setCompressorUnits_{#1}}\xspace}
\newcommand{\setCompressorConfigurations}[1]{\ensuremath{\mathcal{C}_{#1}}\xspace}
\newcommand{\setCompressorConfigurationsUsingUnit}[1]{\ensuremath{\mathcal{C}_{#1}}\xspace}
\newcommand{\setConfigurationFacets}[1]{\ensuremath{\setFacets{#1}}\xspace}

% navi station specific (net model)
\newcommand{\naviStationGraph}[1]{\ensuremath{G}_{#1}\xspace}
\newcommand{\naviStationGraphAll}[1]{\ensuremath{\naviStationGraph{#1}=(\setVerticesNaviStation{#1},\setArtificialLinksNaviStation{#1})}\xspace}
\newcommand{\setVerticesNaviStation}[1]{\ensuremath{\setVertices_{#1}}\xspace}
\newcommand{\setArtificialLinksNaviStation}[1]{\ensuremath{\setArtificialLinks_{#1}}\xspace}
\newcommand{\nNaviStations}{\ensuremath{m}\xspace}
% Felix' net model
\newcommand{\setNetworkStations}{\ensuremath{\mathcal{I}}\xspace} % not sure why we have sets for everything but number the stations???
\newcommand{\setAuxCompressorConfigs}{\ensuremath{\mathcal{C}^\mathrm{ar}}\xspace}
\newcommand{\setAuxCompressorConfigsI}[1]{\ensuremath{\setAuxCompressorConfigs_{#1}}\xspace}
\newcommand{\setAuxCompressorConfigConflicts}{\ensuremath{\mathcal{Z}}\xspace}
\newcommand{\setAuxCompressorConfigConflictsI}[1]{\ensuremath{\setAuxCompressorConfigConflicts_{#1}}\xspace}
\newcommand{\setSimpleStationValidPairs}{\ensuremath{\mathcal{Q}}\xspace} %TODO distinguish from setNSValidPairs below for Felix' diss
\newcommand{\setInitActiveSimpleStates}{\ensuremath{\mathcal{S}^0}\xspace}
\newcommand{\setInitActiveCompressorUnits}{\ensuremath{\mathcal{U}^0}\xspace}
\newcommand{\setInitActiveAuxCompressorConfigs}{\ensuremath{\mathcal{C}^\mathrm{ar0}}\xspace}


% navi station specific (station model)
\newcommand{\setNSModes}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\setNSValidPairs}{\ensuremath{\mathcal{Q}}\xspace} % valid pairs of operation modes and flow directions
\newcommand{\setNSFenceGroups}{\ensuremath{\mathcal{G}}\xspace}
% old commands, deprecated, just used to create the latexdiff for the stationModelPaper
\newcommand{\setOldNSValidPairs}{\ensuremath{\mathcal{OF}}\xspace}
\newcommand{\setOldNSFenceGroups}{\ensuremath{\mathcal{FG}}\xspace}
% end of old commands
\newcommand{\setFenceNodeExitPI}[1]{\ensuremath{\setVertices^\mathrm{fnExP}_{#1}}\xspace}

%%-----------------------------------------------------------
%% Time
%%----------------------------------------------------------
\newcommand{\setTimesteps}{\ensuremath{\mathcal{T}_0}\xspace}
\newcommand{\setTimestepsNoZero}{\ensuremath{\mathcal{T}}\xspace}
\newcommand{\nTimesteps}{\ensuremath{t^\mathrm{max}}\xspace}
\newcommand{\setTimestepsAll}{\ensuremath{\setTimesteps := \{0, \dots, \nTimesteps\}}\xspace}
\newcommand{\setTimestepsNoZeroAll}{\ensuremath{\setTimestepsNoZero := \setTimesteps\setminus\{0\}}\xspace}
\newcommand{\granularity}{\ensuremath{\tau}\xspace}
\newcommand{\granularityI}[1]{\ensuremath{\granularity(#1)}\xspace}

%%-----------------------------------------------------------
%% Supplies and demands
%%----------------------------------------------------------
\newcommand{\inflow}{\ensuremath{d}}
\newcommand{\paramInflowValue}[2]{\ensuremath{D_{#1,#2}}\xspace}
\newcommand{\paramSupplyValue}[2]{\ensuremath{\paramInflowValue{#1}{#2}}\xspace} %TODO Kai: replace by \paramInflowValue
\newcommand{\paramDemandValue}[2]{\ensuremath{\paramInflowValue{#1}{#2}}\xspace} %TODO Kai: replace by \paramInflowValue
\newcommand{\paramSupplyUB}[2]{\ensuremath{\ub{D}_{#1,#2}}\xspace}
\newcommand{\paramDemandUB}[2]{\ensuremath{\lb{D}_{#1,#2}}\xspace}
\newcommand{\inflowI}[1]{\ensuremath{\inflow_{#1}}\xspace}
\newcommand{\paramInflowValueUB}[2]{\ensuremath{\ub{\inflow}_{#1,#2}}\xspace}
\newcommand{\paramInflowValueLB}[2]{\ensuremath{\lb{\inflow}_{#1,#2}}\xspace}
\newcommand{\varSupplyValue}[2]{\ensuremath{\inflowI{#1,#2}}\xspace} %TODO Kai: replace by \inflowI
\newcommand{\varDemandValue}[2]{\ensuremath{\inflowI{#1,#2}}\xspace} %TODO Kai: replace by \inflowI

% station model demands for inflow and pressure
\newcommand{\demandPressure}[1]{\ensuremath{\hat{\press}_{#1}}\xspace}
\newcommand{\demandInflow}[1]{\ensuremath{\hat{\inflow}_{#1}}\xspace}

%%-----------------------------------------------------------
%% Pressure
%%----------------------------------------------------------
\newcommand{\press}{\ensuremath{p}\xspace}
\newcommand{\pressI}[1]{\ensuremath{\press_{#1}}\xspace}
\newcommand{\pressUB}[1]{\ensuremath{\ub{\press}_{#1}}\xspace}
\newcommand{\pressLB}[1]{\ensuremath{\lb{\press}_{#1}}\xspace}
\newcommand{\inflowPressUB}[1]{\ensuremath{\paramPressUB{#1}^{\mathrm{act}}}\xspace} % act => active
\newcommand{\inflowPressLB}[1]{\ensuremath{\paramPressLB{#1}^{\mathrm{act}}}\xspace} % act => active

%%-----------------------------------------------------------
%% Flow
%%----------------------------------------------------------
\newcommand{\mFlow}{\ensuremath{q}\xspace}
\newcommand{\mFlowI}[1]{\ensuremath{\mFlow_{#1}}\xspace}
% Kai's version
%\newcommand{\mFlowFwd}[1]{\ensuremath{\mFlowI{#1}^{\rightarrow}}\xspace}
%\newcommand{\mFlowBwd}[1]{\ensuremath{\mFlowI{#1}^{\leftarrow}}\xspace}
% Felix' version
\newcommand{\mFlowFwdI}[1]{\ensuremath{\mFlowI{#1}^{\mathrm{fwd}}}\xspace}
\newcommand{\mFlowBwdI}[1]{\ensuremath{\mFlowI{#1}^{\mathrm{bwd}}}\xspace}
\newcommand{\mFlowUB}[1]{\ensuremath{\ub{\mFlow}_{#1}}\xspace}
\newcommand{\mFlowLB}[1]{\ensuremath{\lb{\mFlow}_{#1}}\xspace}
\newcommand{\fenceFlow}[1]{\ensuremath{\varArcFlow{#1}^\mathrm{fn}}\xspace}

%%-----------------------------------------------------------
%% Netmodel Navi Station
%%----------------------------------------------------------
\newcommand{\setArtificialLinks}{\ensuremath{\setArcs^{\mathrm{ar}}}\xspace}
\newcommand{\setShortcuts}{\ensuremath{\setArcs^{\mathrm{arSc}}}\xspace}
\newcommand{\setShortcutsNaviStation}[1]{\ensuremath{\setShortcuts_{#1}}\xspace}
\newcommand{\setRegulatorArcs}{\ensuremath{\setArcs^{\mathrm{arRg}}}\xspace}
\newcommand{\setRegulatorArcsNaviStation}[1]{\ensuremath{\setRegulatorArcs_{#1}}\xspace}
\newcommand{\setCompressorArcs}{\ensuremath{\setArcs^{\mathrm{arCp}}}\xspace}
\newcommand{\setCompressorArcsNaviStation}[1]{\ensuremath{\setCompressorArcs_{#1}}\xspace}
\newcommand{\setCombinedArcs}{\ensuremath{\setArcs^{\mathrm{arCb}}}\xspace}
\newcommand{\setCombinedArcsNaviStation}[1]{\ensuremath{\setCombinedArcs_{#1}}\xspace}

% changed by Felix
\newcommand{\setBiRegulatorArcs}{\ensuremath{\setArcs^{\mathrm{arBiRg}}}\xspace}
\newcommand{\setBiRegulatorArcsNaviStation}[1]{\ensuremath{\setBiRegulatorArcs_{#1}}\xspace}
\newcommand{\setBiCompressorArcs}{\ensuremath{\setArcs^{\mathrm{arBiCp}}}\xspace}
\newcommand{\setBiCompressorArcsNaviStation}[1]{\ensuremath{\setBiCompressorArcs_{#1}}\xspace}
\newcommand{\setBiCombinedArcs}{\ensuremath{\setArcs^{\mathrm{arBiCb}}}\xspace}
\newcommand{\setBiCombinedArcsNaviStation}[1]{\ensuremath{\setBiCombinedArcs_{#1}}\xspace}

\newcommand{\setDirectedArcs}{\ensuremath{\setArcs^{\mathrm{ar-di}}}\xspace}
\newcommand{\setDirectedArcsNaviStation}[1]{\ensuremath{\setDirectedArcs_{#1}}\xspace}
\newcommand{\setBiArcs}{\ensuremath{\setArcs^{\mathrm{ar-bi}}}\xspace}
\newcommand{\setBiArcsNaviStation}[1]{\ensuremath{\setBiArcs_{#1}}\xspace}
\newcommand{\setCompressingArcs}{\ensuremath{\setArcs^{\mathrm{ar-co}}}\xspace}
\newcommand{\setCompressingArcsNaviStation}[1]{\ensuremath{\setCompressingArcs_{#1}}\xspace}

\newcommand{\setSimpleStates}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\setSimpleStatesI}[1]{\ensuremath{\setSimpleStates_{#1}}\xspace}
% Kai's version
%\newcommand{\simpleState}{\ensuremath{s}\xspace}
%\newcommand{\simpleStateFlowDirections}{\ensuremath{\simpleState^{\flowDirection}}\xspace}
%\newcommand{\simpleStateLinksActive}{\ensuremath{\simpleState^{on}}\xspace}
%\newcommand{\simpleStateLinksInactive}{\ensuremath{\simpleState^{off}}\xspace}
% Felix' version
\newcommand{\simpStOnArcsI}[1]{\ensuremath{\setArcs^\mathrm{on}_{#1}}\xspace}
\newcommand{\simpStOffArcsI}[1]{\ensuremath{\setArcs^\mathrm{off}_{#1}}\xspace}

\newcommand{\activation}{\ensuremath{x}\xspace}
% Kai's version
%\newcommand{\varActivation}[2]{\ensuremath{\activation_{#1,#2}}\xspace}
%\newcommand{\varFlowDirectionActivation}[2]{\ensuremath{\varActivation{#1}{#2}}\xspace}
%\newcommand{\varSimpleStateActivation}[2]{\ensuremath{\varActivation{#1}{#2}}\xspace}
%\newcommand{\varArtificialLinkActivation}[2]{\ensuremath{\varActivation{#1}{#2}}\xspace}
%\newcommand{\varArtificialLinkActivationFwd}[2]{\ensuremath{\varArtificialLinkActivation{#1}{#2}^{\rightarrow}}\xspace}
%\newcommand{\varArtificialLinkActivationBwd}[2]{\ensuremath{\varArtificialLinkActivation{#1}{#2}^{\leftarrow}}\xspace}
%\newcommand{\varCombinedLinkRegulatingActivation}[2]{\ensuremath{\varArtificialLinkActivation{#1}{#2}^{\mathrm{rg}}}\xspace}
%\newcommand{\varCombinedLinkCompressingActivation}[2]{\ensuremath{\varArtificialLinkActivation{#1}{#2}^{\mathrm{cp}}}\xspace}
% Felix' version ...
\newcommand{\activeArcI}[1]{\ensuremath{x^\mathrm{arc}_{#1}}\xspace}
\newcommand{\activeFwdI}[1]{\ensuremath{x^\mathrm{fwd}_{#1}}\xspace}
\newcommand{\activeBwdI}[1]{\ensuremath{x^\mathrm{bwd}_{#1}}\xspace}
\newcommand{\activeCfgI}[1]{\ensuremath{x^\mathrm{cfg}_{#1}}\xspace}
\newcommand{\activeState}{\ensuremath{x^\mathrm{st}}\xspace}
\newcommand{\activeStateI}[1]{\ensuremath{\activeState_{#1}}\xspace}
\newcommand{\activeFlowDirI}[1]{\ensuremath{x^\mathrm{fd}_{#1}}\xspace}

\newcommand{\varChange}[2]{\ensuremath{\delta_{#1,#2}}\xspace}
\newcommand{\varFlowDirectionChange}[2]{\ensuremath{\varChange{#1}{#2}}\xspace}
\newcommand{\varSimpleStateChange}[2]{\ensuremath{\varChange{#1}{#2}}\xspace}
\newcommand{\varArtificialLinkChangeOn}[2]{\ensuremath{\varChange{#1}{#2}^{\mathrm{on}}}\xspace}
\newcommand{\varArtificialLinkChangeOff}[2]{\ensuremath{\varChange{#1}{#2}^{\mathrm{off}}}\xspace}

\newcommand{\setFlowDirectionConditions}{\ensuremath{\mathcal{W}}\xspace}
\newcommand{\setFlowDirectionConditionsNaviStation}[1]{\ensuremath{\setFlowDirectionConditions_{i}}\xspace}

%%-----------------------------------------------------------
%% Machines, Power, Compression Ratio, and Betriebsvolumenstrom
%%-----------------------------------------------------------
\newcommand{\setMachinesNaviStation}[1]{\ensuremath{\mathcal{M}}_{#1}\xspace}
\newcommand{\setMachinesNaviStationOnLink}[2]{\ensuremath{\setMachinesNaviStation{#1}^{#2}}\xspace}
\newcommand{\generalMachine}{\ensuremath{m}\xspace}
\newcommand{\machine}[1]{\ensuremath{\generalMachine_{#1}}\xspace}

\newcommand{\varAssignMachineToLink}[3]{\ensuremath{y_{#1,#2,#3}}\xspace}

\newcommand{\paramMaxNumberMachinesLink}{\ensuremath{M_a^{\mathrm{max}}}\xspace}
\newcommand{\paramMaxCompressionRatio}[2]{\ensuremath{R_{\machine{#1},#2}}\xspace}
\newcommand{\paramMaxPower}[2]{\ensuremath{\power_{\machine{#1},#2}}\xspace}
\newcommand{\paramMaxBetriebsVolumenstrom}[2]{\ensuremath{\volumetricFlow_{\machine{#1},#2}}\xspace}

\newcommand{\varCompressionRatio}[2]{\ensuremath{r_{#1,#2}}\xspace}
\newcommand{\varPower}[2]{\ensuremath{\pi_{#1,#2}}\xspace}
\newcommand{\varBetriebsVolumenstrom}[2]{\ensuremath{\omega_{#1,#2}}\xspace}
\newcommand{\varMaxPower}[2]{\ensuremath{\varPower{#1}{#2}^{max}}\xspace}
\newcommand{\varMaxBetriebsVolumenstrom}[2]{\ensuremath{\varBetriebsVolumenstrom{#1}{#2}^{max}}\xspace}

\newcommand{\paramMaxCompressionRatioLink}[2]{\ensuremath{\ub{R}_{#1,#2}}\xspace}
\newcommand{\paramPressureUBCompression}[2]{\ensuremath{\paramPressureUB{#1}{#2}^{\mathrm{out}}}\xspace}


%%-----------------------------------------------------------
%% Smoothing
%%-----------------------------------------------------------

\newcommand{\generalSmoothing}{\ensuremath{\delta}\xspace}
\newcommand{\varSmoothingPressurePos}[2]{\ensuremath{\generalSmoothing_{#1,#2}^{\press+}}\xspace}
\newcommand{\varSmoothingPressureNeg}[2]{\ensuremath{\generalSmoothing_{#1,#2}^{\press-}}\xspace}
\newcommand{\varSmoothingInflowPos}[2]{\ensuremath{\generalSmoothing_{#1,#2}^{\mFlow+}}\xspace}
\newcommand{\varSmoothingInflowNeg}[2]{\ensuremath{\generalSmoothing_{#1,#2}^{\mFlow-}}\xspace}

%%-----------------------------------------------------------
%% Flow Direction (used in both models)
%%-----------------------------------------------------------
\newcommand{\setFlowDirections}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\setFlowDirectionsI}[1]{\ensuremath{\setFlowDirections_{#1}}\xspace}
% Kai's and Station model's notation
\newcommand{\flowDirection}{\ensuremath{f}\xspace}
\newcommand{\flowDirectionEntries}{\ensuremath{\flowDirection^{+}}\xspace}
\newcommand{\flowDirectionExits}{\ensuremath{\flowDirection^{-}}\xspace}
\newcommand{\pressUBExitFG}[1]{\ensuremath{\ub{\press}_{#1}^{\mathrm{exit}}}\xspace}
% Felix' new notation
\newcommand{\flowDirEntriesI}[1]{\ensuremath{\setVertices^\mathrm{in}_{#1}}\xspace}
\newcommand{\flowDirExitsI}[1]{\ensuremath{\setVertices^\mathrm{out}_{#1}}\xspace}


%%-----------------------------------------------------------
%% Mode variables
%%----------------------------------------------------------
\newcommand{\mode}{\ensuremath{m}\xspace}
\newcommand{\modeOp}[1]{\ensuremath{\mode_{#1}^\mathrm{op}}\xspace}
\newcommand{\modeCl}[1]{\ensuremath{\mode_{#1}^\mathrm{cl}}\xspace}
\newcommand{\modeBy}[1]{\ensuremath{\mode_{#1}^\mathrm{by}}\xspace}
\newcommand{\modeAc}[1]{\ensuremath{\mode_{#1}^\mathrm{ac}}\xspace}
\newcommand{\modeCv}[1]{\ensuremath{\mode_{#1}^\mathrm{cvcl}}\xspace} % closed because of a check valve
\newcommand{\modeFix}[1]{\ensuremath{\mode_{#1}^\mathrm{fix}}\xspace} % fixed mode for non-controllable regulators
\newcommand{\modeX}[1]{\ensuremath{\mode_{#1}^\mathrm{x}}\xspace}
\newcommand{\cfg}[1]{\ensuremath{\mode_{#1}^\mathrm{cf}}\xspace}
\newcommand{\opMode}[1]{\ensuremath{\mode_{#1}^\mathrm{om}}\xspace}
\newcommand{\flowDir}[1]{\ensuremath{\mode_{#1}^\mathrm{fd}}\xspace}


%%-----------------------------------------------------------
%% Mode specific pressure and flow variables
%%----------------------------------------------------------
\newcommand{\pressBy}[1]{\ensuremath{\pressI{#1}^\mathrm{by}}\xspace}
\newcommand{\mFlowBy}[1]{\ensuremath{\mFlowI{#1}^\mathrm{by}}\xspace}
\newcommand{\pressClL}[1]{\ensuremath{\pressI{#1}^\mathrm{l-cl}}\xspace}
\newcommand{\pressClR}[1]{\ensuremath{\pressI{#1}^\mathrm{r-cl}}\xspace}
% there is no closed flow, it's zero
\newcommand{\pressCfgL}[1]{\ensuremath{\pressI{#1}^\mathrm{l-cf}}\xspace}
\newcommand{\pressCfgR}[1]{\ensuremath{\pressI{#1}^\mathrm{r-cf}}\xspace}
\newcommand{\mFlowCfg}[1]{\ensuremath{\mFlowI{#1}^\mathrm{cf}}\xspace}
%% upper bounds for all of them
\newcommand{\pressByUB}[1]{\ensuremath{\pressUB{#1}^\mathrm{by}}\xspace}
\newcommand{\mFlowByUB}[1]{\ensuremath{\mFlowUB{#1}^\mathrm{by}}\xspace}
\newcommand{\pressClLUB}[1]{\ensuremath{\pressUB{#1}^\mathrm{l-cl}}\xspace}
\newcommand{\pressClRUB}[1]{\ensuremath{\pressUB{#1}^\mathrm{r-cl}}\xspace}
% there is no closed flow, it's zero
\newcommand{\pressCfgLUB}[1]{\ensuremath{\pressUB{#1}^\mathrm{l-cf}}\xspace}
\newcommand{\pressCfgRUB}[1]{\ensuremath{\pressUB{#1}^\mathrm{r-cf}}\xspace}
\newcommand{\mFlowCfgUB}[1]{\ensuremath{\mFlowUB{#1}^\mathrm{cf}}\xspace}
%% lower bounds for all of them
\newcommand{\pressByLB}[1]{\ensuremath{\pressLB{#1}^\mathrm{by}}\xspace}
\newcommand{\mFlowByLB}[1]{\ensuremath{\mFlowLB{#1}^\mathrm{by}}\xspace}
\newcommand{\pressClLLB}[1]{\ensuremath{\pressLB{#1}^\mathrm{l-cl}}\xspace}
\newcommand{\pressClRLB}[1]{\ensuremath{\pressLB{#1}^\mathrm{r-cl}}\xspace}
% there is no closed flow, it's zero
\newcommand{\pressCfgLLB}[1]{\ensuremath{\pressLB{#1}^\mathrm{l-cf}}\xspace}
\newcommand{\pressCfgRLB}[1]{\ensuremath{\pressLB{#1}^\mathrm{r-cf}}\xspace}
\newcommand{\mFlowCfgLB}[1]{\ensuremath{\mFlowLB{#1}^\mathrm{cf}}\xspace}

%%-----------------------------------------------------------
%% Slack variables
%%----------------------------------------------------------
\newcommand{\slack}{\ensuremath{\sigma}\xspace}
\newcommand{\slackPPos}[1]{\ensuremath{\slack_{#1}^{\press+}}\xspace}
\newcommand{\slackPNeg}[1]{\ensuremath{\slack_{#1}^{\press-}}\xspace}
\newcommand{\slackQPos}[1]{\ensuremath{\slack_{#1}^{\inflow+}}\xspace}
\newcommand{\slackQNeg}[1]{\ensuremath{\slack_{#1}^{\inflow-}}\xspace}
\newcommand{\slackPUB}{\ensuremath{\ub{\slack}^{\press}}\xspace}
\newcommand{\slackQUB}{\ensuremath{\ub{\slack}^{\inflow}}\xspace}

%%-----------------------------------------------------------
%% Target values
%%----------------------------------------------------------
%% target value types
\newcommand{\PIN}{\pressI{\ell}\xspace}
\newcommand{\POUT}{\pressI{r}\xspace}
\newcommand{\MINPIN}{\ensuremath{\underbracket[0.1ex][0.22ex]{\,\PIN\,}}\xspace}
\newcommand{\MAXPIN}{\ensuremath{\overbracket[0.1ex][0.22ex]{\,\PIN\,}}\xspace}
\newcommand{\MINPOUT}{\ensuremath{\underbracket[0.1ex][0.22ex]{\,\POUT\,}}\xspace}
\newcommand{\MAXPOUT}{\ensuremath{\overbracket[0.1ex][0.22ex]{\,\POUT\,}}\xspace}
\newcommand{\MINQ}{\ensuremath{\underbracket[0.1ex][0.22ex]{\,\mFlow\,}}\xspace}
\newcommand{\MAXQ}{\ensuremath{\overbracket[0.1ex][0.22ex]{\,\mFlow\,}}\xspace}
\newcommand{\SETQ}{\ensuremath{\mFlowI{\mathrm{set}}}\xspace}

%% sets
\newcommand{\setTargetValues}{\ensuremath{\Gamma}\xspace} % all TVs
\newcommand{\setTargetValuesI}[1]{\ensuremath{\setTargetValues_{#1}}\xspace} % ... of some element
\newcommand{\setStaPush}{\ensuremath{\Theta}\xspace} % all stable/pushing TV combinations
\newcommand{\setStaPushI}[1]{\ensuremath{\setStaPush_{#1}}\xspace} % ... of some element
\newcommand{\setStaPushActive}{\ensuremath{\setStaPush^\mathrm{ac}}\xspace} % all combinations for active mode
\newcommand{\setStaPushActiveI}[1]{\ensuremath{\setStaPushActive_{#1}}\xspace} % ... of some element
\newcommand{\setStaPushOpen}{\ensuremath{\setStaPush^\mathrm{op}}\xspace} % all combinations for open mode
\newcommand{\setStaPushOpenI}[1]{\ensuremath{\setStaPushOpen_{#1}}\xspace} % ... of some element
\newcommand{\setStaPushClosed}{\ensuremath{\setStaPush^\mathrm{cl}}\xspace} % all combinations for closed mode
\newcommand{\setStaPushClosedI}[1]{\ensuremath{\setStaPushClosed_{#1}}\xspace} % ... of some element
\newcommand{\setStaPushXI}[1]{\ensuremath{\setStaPush^\mathrm{x}_{#1}}\xspace} % all combination for x mode for some element
\newcommand{\setTVBPolysI}[1]{\ensuremath{\Phi_{#1}}\xspace}
\newcommand{\setTVBPolysActiveI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{ac}}\xspace}
\newcommand{\setTVBPolysBypassI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{by}}\xspace}
\newcommand{\setTVBPolysClosedI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{cl}}\xspace}
\newcommand{\setTVBPolysActiveQI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{ac\text{-}Q}}\xspace}
\newcommand{\setTVBPolysActivePInI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{ac\text{-}p_{in}}}\xspace}
\newcommand{\setTVBPolysActivePOutI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{ac\text{-}p_{out}}}\xspace}
\newcommand{\setTVBPolysActiveXI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{ac\text{-}X}}\xspace}
\newcommand{\setTVBPolysXI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{X}}\xspace}
\newcommand{\setTVQuantities}{\ensuremath{\Omega}\xspace}

%% vars
\newcommand{\tv}{\ensuremath{\tau}\xspace}
\newcommand{\tvI}[1]{\ensuremath{\tv_{#1}}\xspace}
\newcommand{\lbTVI}[1]{\ensuremath{\lb{\tv}_{#1}}\xspace}
\newcommand{\ubTVI}[1]{\ensuremath{\ub{\tv}_{#1}}\xspace}

% set values

\newcommand{\tvSet}{\ensuremath{\tv^\mathrm{set}}\xspace}
\newcommand{\tvSetI}[1]{\ensuremath{\tvSet_{#1}}\xspace}

% target value bound polytope variable
\newcommand{\tvPolyI}[1]{\ensuremath{\phi_{#1}}\xspace}

% target value stable pushing combination variable
\newcommand{\tvCombi}{\ensuremath{\theta}\xspace}
\newcommand{\tvCombiI}[1]{\ensuremath{\tvCombi_{#1}}\xspace}
\newcommand{\funcTvPrio}{\ensuremath{\varphi}\xspace} % target value priority function
\newcommand{\funcTvPrioI}[1]{\ensuremath{\funcTvPrio(#1)}\xspace} % .. with argument


%%-----------------------------------------------------------
%% Objective change variables
%%----------------------------------------------------------
\newcommand{\objVar}{\ensuremath{\delta}\xspace}
\newcommand{\objVarI}[1]{\ensuremath{\delta_{#1}}\xspace}
\newcommand{\opModeChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{om}}}\xspace}
\newcommand{\unitStart}[1]{\ensuremath{\objVarI{#1}^{\mathrm{us}}}\xspace}
\newcommand{\regModeChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{rg}}}\xspace}
\newcommand{\xPLChg}[1]{\ensuremath{\objVarI{#1}^{\text{X-pl}}}\xspace}
\newcommand{\xPRChg}[1]{\ensuremath{\objVarI{#1}^{\text{X-pr}}}\xspace}
\newcommand{\xQChg}[1]{\ensuremath{\objVarI{#1}^{\text{X-q}}}\xspace}
\newcommand{\rgPLChg}[1]{\ensuremath{\objVarI{#1}^{\text{rg-pl}}}\xspace}
\newcommand{\rgPRChg}[1]{\ensuremath{\objVarI{#1}^{\text{rg-pr}}}\xspace}
\newcommand{\rgQChg}[1]{\ensuremath{\objVarI{#1}^{\text{rg-qa}}}\xspace}
\newcommand{\rgYChg}[1]{\ensuremath{\objVarI{#1}^{\text{rg-y}}}\xspace}
\newcommand{\csPLChg}[1]{\ensuremath{\objVarI{#1}^{\text{cs-pl}}}\xspace}
\newcommand{\csPRChg}[1]{\ensuremath{\objVarI{#1}^{\text{cs-pr}}}\xspace}
\newcommand{\csQChg}[1]{\ensuremath{\objVarI{#1}^{\text{cs-qa}}}\xspace}
\newcommand{\tvChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{tv}}}\xspace}
\newcommand{\tvSetChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{set}}}\xspace}
% new changes in Felix' netmodel
\newcommand{\valveModeChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{va}}}\xspace}
\newcommand{\auxArcActivityChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{arc}}}\xspace}
\newcommand{\simpleStateTurnOn}[1]{\ensuremath{\objVarI{#1}^{\mathrm{st}}}\xspace}
\newcommand{\fnPChg}[1]{\ensuremath{\objVarI{#1}^{\text{fn-p}}}\xspace}
\newcommand{\fnQChg}[1]{\ensuremath{\objVarI{#1}^{\text{fn-q}}}\xspace}

%%-----------------------------------------------------------
%% Objective cost parameters
%%-----------------------------------------------------------
\newcommand{\cost}{\ensuremath{w}\xspace}
\newcommand{\costSlackP}{\ensuremath{\cost^{\slack\text{-p}}}\xspace}
\newcommand{\costSlackQ}{\ensuremath{\cost^{\slack\text{-d}}}\xspace}
\newcommand{\costOpModes}{\ensuremath{\cost^\mathrm{om}}\xspace}
\newcommand{\costUnitStarts}{\ensuremath{\cost^\mathrm{us}}\xspace}
\newcommand{\costVaModeChg}{\ensuremath{\cost^\mathrm{va}}\xspace}
\newcommand{\costRgModeChg}{\ensuremath{\cost^\mathrm{rg}}\xspace}
\newcommand{\costXPLChg}{\ensuremath{\cost^\text{X-pl}}\xspace}
\newcommand{\costXPRChg}{\ensuremath{\cost^\text{X-pr}}\xspace}
\newcommand{\costXQChg}{\ensuremath{\cost^\text{X-q}}\xspace}
\newcommand{\costRgPLChg}{\ensuremath{\cost^\text{rg-pl}}\xspace}
\newcommand{\costRgPRChg}{\ensuremath{\cost^\text{rg-pr}}\xspace}
\newcommand{\costRgQChg}{\ensuremath{\cost^\text{rg-q}}\xspace}
\newcommand{\costCsPLChg}{\ensuremath{\cost^\text{cs-pl}}\xspace}
\newcommand{\costCsPRChg}{\ensuremath{\cost^\text{cs-pr}}\xspace}
\newcommand{\costCsQChg}{\ensuremath{\cost^\text{cs-q}}\xspace}
\newcommand{\costFlowDirectionChange}{\ensuremath{\cost^f}\xspace}
\newcommand{\costFlowDirectionChangeNaviStation}[1]{\ensuremath{\costFlowDirectionChange_{#1}}\xspace}
\newcommand{\costOriginalSimpleStateChange}{\ensuremath{\tilde{\cost}^\mathrm{st}}\xspace}
\newcommand{\costSimpleStateChangeI}[1]{\ensuremath{\cost^\mathrm{st}_{#1}}\xspace}
\newcommand{\costArtificialLinkChange}{\ensuremath{\cost^\mathrm{arc}}\xspace}
\newcommand{\costCompressingLinkOn}[1]{\ensuremath{\cost_{#1}^{\text{cp-act}}}\xspace}
\newcommand{\costCompressingLinkValue}[1]{\ensuremath{\cost_{#1}^{\text{cp-val}}}\xspace}
\newcommand{\costSmoothingPressure}{\ensuremath{\cost^{\text{sm-p}}}\xspace}
\newcommand{\costSmoothingFlow}{\ensuremath{\cost^{\text{sm-q}}}\xspace}
\newcommand{\costTVChg}{\ensuremath{\cost^\mathrm{tv}}\xspace}
\newcommand{\costUnitRunning}{\ensuremath{\cost^\mathrm{ru}}\xspace}
\newcommand{\costFenceNodePChg}{\ensuremath{\cost^\text{fn-p}}\xspace}
\newcommand{\costFenceNodeQChg}{\ensuremath{\cost^\text{fn-q}}\xspace}

%%-----------------------------------------------------------
%% Other physical quantities
%%----------------------------------------------------------
\newcommand{\velo}{\ensuremath{v}\xspace}
\newcommand{\absVelo}[1]{\ensuremath{|\velo_{#1}|}\xspace}
\newcommand{\gasConst}{\ensuremath{R}\xspace}
\newcommand{\sGasConst}{\ensuremath{\gasConst_{\mathrm{s}}}\xspace}
\newcommand{\temp}{\ensuremath{T}\xspace}
\newcommand{\tempI}[1]{\ensuremath{\temp_{#1}}\xspace}
\newcommand{\zFact}{\ensuremath{z}\xspace}
\newcommand{\zFactI}[1]{\ensuremath{\zFact_{#1}}\xspace}
\newcommand{\vol}{\ensuremath{V}\xspace}
\newcommand{\amountOfSubstance}{\ensuremath{n}\xspace}
\newcommand{\pseudoP}{\ensuremath{\press^\mathrm{c}}\xspace}
\newcommand{\pseudoT}{\ensuremath{\temp^\mathrm{c}}\xspace}
\newcommand{\molMass}{\ensuremath{M}\xspace}
\newcommand{\len}{\ensuremath{L}\xspace}
\newcommand{\lenI}[1]{\ensuremath{\len_{#1}}\xspace}
\newcommand{\area}{\ensuremath{A}\xspace}
\newcommand{\areaI}[1]{\ensuremath{\area_{#1}}\xspace}
\newcommand{\diam}{\ensuremath{D}\xspace}
\newcommand{\diamI}[1]{\ensuremath{\diam_{#1}}\xspace}
\newcommand{\slope}{\ensuremath{s}\xspace}
\newcommand{\slopeI}[1]{\ensuremath{\slope_{#1}}\xspace}
\newcommand{\fric}{\ensuremath{\lambda}\xspace}
\newcommand{\fricI}[1]{\ensuremath{\fric_{#1}}\xspace}
\newcommand{\rough}{\ensuremath{k}\xspace}
\newcommand{\roughI}[1]{\ensuremath{\rough_{#1}}\xspace}
\newcommand{\dynVisc}{\ensuremath{\eta}\xspace}
\newcommand{\gravAcc}{\ensuremath{g}\xspace}
\newcommand{\dens}{\ensuremath{\rho}\xspace}
\newcommand{\densI}[1]{\ensuremath{\dens_{#1}}\xspace}
\newcommand{\nDensLow}{\ensuremath{\dens_0}\xspace} % subscript is used in the inertial term paper as \nDens^\text{max} for this and should be left free, if possible ... where?
\newcommand{\nDens}{\ensuremath{\dens^0}\xspace}
\newcommand{\vFlow}{\ensuremath{Q}\xspace}
\newcommand{\vFlowI}[1]{\ensuremath{\vFlow_{#1}}\xspace}
\newcommand{\nvFlow}{\ensuremath{Q^0}\xspace}
\newcommand{\nvFlowI}[1]{\ensuremath{\nvFlow_{#1}}\xspace}
\newcommand{\timeDiff}{\ensuremath{\Delta_t}\xspace} %equals \tau(t) - \tau(t-1)
\newcommand{\power}{\ensuremath{P}\xspace}
\newcommand{\powerI}[1]{\ensuremath{\power_{#1}}\xspace}
\newcommand{\adEnth}{\ensuremath{H_\mathrm{ad}}\xspace}
\newcommand{\adEff}{\ensuremath{\eta_\mathrm{ad}}\xspace} % \eta is already the dyn viscosity, but it's the same in the gas book
\newcommand{\isenExp}{\ensuremath{\kappa}\xspace}
\newcommand{\pRatio}{\ensuremath{\psi}\xspace}
\newcommand{\pRatioI}[1]{\ensuremath{\pRatio_{#1}}\xspace}

%%-----------------------------------------------------------
%% Other element parameters
%%----------------------------------------------------------
\newcommand{\height}{\ensuremath{h}\xspace}
\newcommand{\heightI}[1]{\ensuremath{\height_{#1}}\xspace}
\newcommand{\dragI}[1]{\ensuremath{\zeta_{#1}}\xspace}
\newcommand{\machinePDiffUB}{\ensuremath{\ub{\Delta}_\press}\xspace}

%%-----------------------------------------------------------
%% Number sets
%%----------------------------------------------------------
\newcommand{\setReals}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\setRealsNonNeg}{\ensuremath{\setReals_{\geq 0}}\xspace}
\newcommand{\setRealsNonPos}{\ensuremath{\setReals_{\leq 0}}\xspace}
\newcommand{\setRealsNeg}{\ensuremath{\setReals_{< 0}}\xspace}
\newcommand{\setRealsPos}{\ensuremath{\setReals_{> 0}}\xspace}
\newcommand{\setNaturalNumbers}{\ensuremath{\mathbb{N}}\xspace}
